Modeling the Location Selection of Mirror Servers in Content Delivery Networks

For a provider of a Content Delivery Network (CDN), the location selection of mirror servers is a complex optimization problem. Generally, the objective is to place the nodes centralized such that all customers have convenient access to the service according to their demands. It is an instance of the k-center problem, which is proven to be NP-hard. Determining reasonable server locations directly influences run time effects and future service costs. We model, simulate, and optimize the properties of a content delivery network. Specifically, considering the server locations in a network infrastructure with prioritized customers and weighted connections. A simulation model for the servers is necessary to analyze the caching behavior in accordance to the targeted customer requests. We analyze the problem and compare different optimization strategies. For our simulation, we employ various realistic scenarios and evaluate several performance indicators. Our new optimization approach shows a significant improvement. The presented results are generally applicable to other domains with k-center problems, e.g., the placement of military bases, the planning and placement of facility locations, or data mining.

==> README <==

March 5, 2007


IEEEtran is the official LaTeX class for authors of the Institute of
Electrical and Electronics Engineers (IEEE) transactions journals and
conferences. The latest version of the IEEEtran package can be found
at CTAN:

http://www.ctan.org/tex-archive/macros/latex/contrib/IEEEtran/

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/


Version 1.7a is a bug fix release that corrects the two column peer
review title page problem. This problem was not present in the 1.6 series.


V1.7 is a significant update over the 1.6 series with many important
changes. For a full list, please read the file changelog.txt. The most
notable changes include:

 1. New class option compsoc to support the IEEE Computer Society format.

 2. Several commands and environments have been deprecated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow the use of
    the obsolete forms (for now), but with a warning message to the console
    during compilation:
    \IEEEauthorblockA, \IEEEauthorblockN, \IEEEauthorrefmark,
    \IEEEbiography, \IEEEbiographynophoto, \IEEEkeywords, \IEEEPARstart,
    \IEEEproof, \IEEEpubid, \IEEEpubidadjcol, \IEEEQED, \IEEEQEDclosed,
    \IEEEQEDopen, \IEEEspecialpapernotice. IEEEtran.cls now redefines
    \proof in way to avoid problems with the amsthm.sty package.
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
    These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. New \CLASSINPUT, \CLASSOPTION and \CLASSINFO interface allows for more
    user control and conditional compilation.

 4. Several bug fixes and improved compatibility with other packages.


A note to those who create classes derived from IEEEtran.cls: Consider the
use of patch code, either in an example .tex file or as a .sty file,
rather than creating a new class. The IEEEtran.cls CLASSINPUT interface
allows IEEEtran.cls to be fully programmable with respect to document
margins, so there is no need for new class files just for altered margins.
In this way, authors can benefit from updates to IEEEtran.cls and the need
to maintain derivative classes and backport later IEEEtran.cls revisions
thereto is avoided. As always, developers who create classes derived from
IEEEtran.cls should use a different name for the derived class, so that it
cannot be confused with the official/base version here, as well as provide
authors with technical support for the derived class. It is generally a bad
idea to produce a new class that is not going to be maintained.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for conference papers.

bare_jrnl.tex          - A bare bones starter file for journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_jrnl.tex, bare_jrnl_compsoc.tex
***************************************************************************


==> content/requirements.tex <==
\section{REQUIREMENTS}\label{sec:requirements}
Before we can optimize the placement of mirror servers and the customer assignment for a specific scenario, we need to know the precise network infrastructure and the connected customers. Therefore, a transformation is necessary from the real network infrastructure to our model. Furthermore, it is mandatory to define the goal of the placement. Typical objective functions include: maximum, quantile 95\% and median as well as average distance of all customers distance to their nearest mirror server. Another popular and highly relevant objective for the management of a CDN providers is a function that tests whether all distances are smaller than a specified limit, to guarantee a certain quality.

Beside these metrics for the optimization, it is important to know general aspects for a provider. Before a concrete planning of the service can take place, the number of corresponding server need to be analyzed to achieve the objective. These locations for servers need to be planned against realistic conditions. A corresponding flexible and powerful optimization algorithm is necessary for this.

%Neben diesen Metriken für die Optimierung ist es für einen Provider wichtig allgemeine Kennzahlen zu wissen. Bevor eine konkrete Planung des Dienstes stattfinden kann, ist unter anderem die Anzahl der entsprechenden Server festzulegen. Diese Standorte für Server sind anhand realistischer Bedingungen zu planen. Ein entsprechende flexibler und leistungsfähiger Optimierungsalgorithmus ist dafür notwendig.

In our work, we analyze the placement concerning to the following aspects:
\begin{itemize}
\item Decision on a meaningful evaluation measure. 
%\item Performance differences between the constraint free and the node placement.
\item Recommended quantity of storage servers in relation to the number of customers and their distance.
\item Fast and adaptable placement algorithms for realistic conditions for the extension of an existing CDN.
\item Meta-Optimization to identify the necessary number of storage servers for a specific scenario to reach a predefined quality.
\end{itemize}





==> content/simulation_and_evaluation.tex <==
\section{SIMULATION AND ASSESSMENT}\label{simulation}
The simulation of the model and the entire system is based on experiments using a prototypic implementation in Java. For the evaluation, we run multiple simulations and compare different optimization algorithms. We used classical geo-coordinates in the 2-dimensional space and the described hop distance combined with euclidean distance as metric. A scenario can be stored and load via XML. The customers, servers, and assignments of customers to nearest servers of a scenarios were visualized via the data format GeoJson \cite{geojson} in TileMill \cite{tilemill}. For the evaluation, the fitness function calculate the distance parameter: maximum, quantile 95\%, median and average. To generate significant findings we performed repeated optimizations using various scenarios from \textit{the internet topology zoo} \cite{Knight2011}. Table \ref{test-setups} show the parameter of the test setups. The achieved results are the average values for each algorithm. 

\begin{table} [htbp]
\begin{center} 
\caption{Parameters of test setups. }
\label{test-setups}

\begin{tabular}{|l!{\vrule width 1.0pt}r|}
\hline
\multicolumn{2}{|c|}{Test Setups} \\
\hline
\hhline{--}
Nodes & 100-1000\\
\hline
%Repetitions & 2\\
%\hline
Scenarios & 10\\
\hline
Servers & 10,20,30\\
\hline
\end{tabular}
\end{center}
\end{table}

 % 1----------------------------------
Initially a Monte Carlo approach for free placement and node placement served as a basic benchmark. Figure \ref{2approx} shows that the 2-Approx algorithms on average returns much better results. Monte Carlo with free placement generated solutions, that were unreliable and too far away from the objective. Therefore it was not a reasonable reference.
For our further evaluation we used the 2-Approx as a reference. Figure \ref{2approx} also illustrates that the average distance to servers is basically meaningless, for the upcoming experiments we focus on the maximum distance as fitness function. Based on the results $s$ of the 2-Approx we defined a theoretical limit for the optimum:    
\begin{equation}
 s \leq 2 \cdot Optimum_{ real} \implies Optimum_{ theoretical} \geq \frac{ 1 }{ 2 } \cdot s
\end{equation}
\begin{figure}[htb]
 {
 \centering
 \includegraphics[width=0.5\textwidth]{fig/2approx.png}
  \caption{Comparison of Monte Carlo and 2-Approx.}
 \label{2approx}
 }
\end{figure}
The solutions of 2-Approx vary because of the random initialization. But anyway, the 2-approximable condition is valid every run.

Figure \ref{DeviationToTheorecticalOptimum} shows the results of algorithm comparison. For small server numbers, our improved Conny algorithm is close to the theoretical optimum. Also the evolutionary heuristic of the framework SEREIN achieves very good results. For larger server counts both algorithms stagnate with their performance nearly at the same level, indicating that we are already very close to the actual optimum. Both approaches performed significantly better than 2-Approx and were much faster than a brute force approach.

  \begin{figure}[htb]
   {
   \centering
   \includegraphics[width=0.5\textwidth]{fig/DeviationToTheorecticalOptimum.png}
   \caption{Deviation between 2-Approx and our best algorithms for maximum distance.}
   \label{DeviationToTheorecticalOptimum}
   }
   \end{figure}

  
 Figure \ref{ComparisonFreeAndNodePlacement} presents the difference between free placement and node placement for our improved algorithm Conny. We observed that the node placement approach would on average need 12\% more servers to compensate for the more flexible positioning of the free placement. In the worst case 16\% more servers were required. While additional servers have a positive effect, increasing the overall capacity and load balance, the added benefit decreases significantly for large server counts. For high ratios of servers in relation to customer count we observe a saturation effect.
 
  \begin{figure}[htb]
  {
  \centering
  \includegraphics[width=0.5\textwidth]{fig/ComparisonFreeAndNodePlacement.png}
  \caption{Deviation between free and node Placement for maximum distance and quantile 95\%.}
  \label{ComparisonFreeAndNodePlacement}
  }
  \end{figure}
    % 2----------------------------------
    
    
    % 4----------------------------------
Based on the maximum distance of a customer to his nearest mirror server, Table \ref{tab:PerformanceComparisonMax} and Figure \ref{fig:PerformanceComparisonMax} show that it is sufficient to set up about at 6\% of the consumer a server. After we placed 58 mirror server for 1.000 customers, the average improvement of maximum distance for an additional server is less than 1\% with the 2-Approx or Conny algorithms.
% We also analyzed this aspect for different customer quantities. The direct number of servers is nearly the same. So we know that this is not directly dependend from the number of customers. It depends also on the size of the area (bounding box), where the customers are placed and the degree of satiation level.

  \begin{figure}[htb]
   {
   \centering
   \includegraphics[width=0.5\textwidth]{fig/PerformanceComparisonMax.png}
   \caption{Performance overview for 1.000 customers. The red vertical line marks the quantity of mirror server, after which the average performance improvement is less than 1\%.}
   \label{fig:PerformanceComparisonMax}
   }
   \end{figure}
\vspace{4mm}



%\begin{table} [htbp]
%\begin{center} 
%\caption{Improvement of maximum distance in relation to number of storage server (2-Approx). }
%\label{tab:PerformanceComparisonMax}
%\begin{tabular}{|c|c|c|}
%\hline
%Storage Server & Distance - Maximum & Improvement in \%\\
%\hline
%\hhline{--}
%10 & 80,0281 & -\\
%\hline
%50 &  29,9952 & 62,5 \\
%\hline
%100 & 19,5603 & 34,8 \\
%\hline
%200 & 12,7547 & 34,8 \\
%\hline
%\end{tabular}
%\end{center}
%\end{table}


%http://www.tablesgenerator.com/latex_tables#
\begin{table} [htbp]
\begin{center} 
\caption{Improvement of maximum distance in relation to number of storage server (2-Approx). }
\label{tab:PerformanceComparisonMax}
\begin{tabular}{|c|c|c|}
\hline
2-Approx & Distance - Maximum & Improvement in \% \\ \hline
 \hhline{---}
1        & 295,7           & -                 \\ \hline
2        & 189,9           & 35,8       \\ \hline
5        & 116,8          & 38,5       \\ \hline
10       & 80,0            & 31,5       \\ \hline
20       & 53,7            & 32,9        \\ \hline
30       & 40,0            & 25,5       \\ \hline
40       & 33,9            & 15,6         \\ \hline
50       & 30,0            & 11,5       \\ \hline
60       & 26,5             & 11,7       \\ \hline
70       & 24,3            & 8,2      \\ \hline
80       & 22,4            & 7,8       \\ \hline
90       & 21,0            & 6,3       \\ \hline
100      & 19,6            & 6,9       \\ \hline
150      & 15,4            & 21,3       \\ \hline
200      & 12,8            & 17,1       \\ \hline
\end{tabular}
\end{center}
\end{table}

    % 4----------------------------------
    
    Figure \ref{fig:PerformanceComparisonMax} and Table \ref{tab:PerformanceOverview} present the general Performance of the different algorithms. The performance of the SEREIN framework with an evolutionary algorithms is remarkably. SEREIN is not customized for this problem but reaches a comparably good solution as the other algorithms specially developed for this task. The parameters of the heuristic were adapted after as little as 6 small test runs. The Performance of the algorithms MacQueen, Lloyd and k-Means++ are nearly the same, so we took the best one of the three, MacQueen. The calculation time of all algorithms depends strongly on their parameters and predefined time limits. The time complexity of the algorithms is widely different, but all optimizations finished after a couple of hours. For such a fundamental decision of mirror placements, the computation time is acceptable.
    
%     \begin{figure}[htb]
%       {
%       \centering
%       \includegraphics[width=0.5\textwidth]{fig/GeneralPerformance.png}
%       \caption{Performance overview.}
%       \label{fig:GeneralPerformance}
%       }
%       \end{figure}


\begin{table} [htbp]
\begin{center} 
\caption{Performance overview with objective maximum distance in relation to number of storage servers. }
\label{tab:PerformanceOverview}
\setlength{\tabcolsep}{4pt}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
\rotatebox{90}{Server} & \rotatebox{90}{Monte Carlo (free)} & \rotatebox{90}{Monte Carlo (node) \text{ }} & \rotatebox{90}{Greedy (node)} & \rotatebox{90}{2-Approx (node)} & \rotatebox{90}{MacQueen (free)} & \rotatebox{90}{Serein (free)} & \rotatebox{90}{Conny (free)} & \rotatebox{90}{Conny (node)} \\ \hline
 \hhline{---------}
1      & 331,2              & 295,7              & 198,3         & 295,7           & 199,7            & 195,9         & 195,9        & 198,3        \\ \hline
2      & 230,9              & 217,2              & 194,6         & 189,9           & 126,2            & 124,6         & 123,7        & 126,6        \\ \hline
5      & 132,1              & 153,3              & 143,8         & 116,8           & 103,4            & 94,0          & 91,7         & 92,9         \\ \hline
10     & 113,2              & 134,5              & 105,0         & 80,0            & 62,4             & 62,5          & 57,4         & 60,0         \\ \hline
20     & 100,0              & 85,8               & 92,7          & 53,7            & 46,6             & 50,8          & 40,3         & 43,2         \\ \hline
30     & 85,4               & 71,4               & 85,3          & 40,0            & 38,9             & 42,3          & 32,8         & 34,8         \\ \hline
40     & 85,2               & 60,2               & 78,8          & 33,9            & 34,2             & 36,4          & 28,4         & 31,8         \\ \hline
50     & 79,0               & 52,6               & 72,5          & 30,0            & 31,3             & 34,1          & 25,6         & 28,3         \\ \hline
60     & 61,3               & 48,4               & 66,7          & 26,5            & 29,1             & 30,9          & 22,7         & 25,9         \\ \hline
70     & 50,8               & 46,0               & 61,3          & 24,3            & 26,8             & 29,3          & 21,2         & 23,5         \\ \hline
80     & 48,9               & 44,5               & 56,7          & 22,4            & 25,5             & 27,9          & 19,5         & 22,0         \\ \hline
90     & 43,0               & 42,9               & 52,3          & 21,0            & 23,5             & 26,9          & 18,4         & 20,8         \\ \hline
100    & 41,1               & 41,3               & 49,1          & 19,6            & 23,0             & 25,9          & 17,1         & 20,1         \\ \hline
150    & 30,7               & 33,7               & 36,4          & 15,4            & 20,1             & 21,7          & 13,6         & 15,6         \\ \hline
200    & 28,2               & 29,6               & 27,5          & 12,8            & 17,0             & 17,6          & 11,4         & 13,1         \\ \hline
\end{tabular}
\end{center}
\end{table}


\vspace{-2mm}
\begin{figure}[htb]
{
\centering
\includegraphics[width=0.48\textwidth]{IndienCombined0.png}
\caption{Example of a scenario in India for the placement of Mirror Server.}
\label{geographical}
}
\end{figure}
\vspace{-4mm}
    
